Offline Policy Optimization with Eligible Actions

Offline policy optimization could have a large impact on many real-world decision-making problems, as online learning may be infeasible in many applications. Importance sampling and its variants are a commonly used type of estimator in offline policy evaluation, and such estimators typically do not require assumptions on the properties and representational capabilities of value function or decision process model function classes. In this paper, we identify an important overfitting phenomenon in optimizing the importance weighted return, in which it may be possible for the learned policy to essentially avoid making aligned decisions for part of the initial state space. We propose an algorithm to avoid this overfitting through a new per-state-neighborhood normalization constraint, and provide a theoretical justification of the proposed algorithm. We also show the limitations of previous attempts to this approach. We test our algorithm in a healthcare-inspired simulator, a logged dataset collected from real hospitals and continuous control tasks. These experiments show the proposed method yields less overfitting and better test performance compared to state-of-the-art batch reinforcement learning algorithms.

==> back_al.tex <==
One might hope that existing methods are sufficient to address this challenge. Here we expand on the discussion in the related work to suggestion why this is not the case. First, 

\textbf{Performance on a validation set}. One reasonable approach when a simulator is unavailable, is to divide the dataset into a training and validation  set. Multiple policies can be trained on the training dataset, and then one policy can be selected based on its estimated performance on the validation set(see e.g.~\cite{thomas2015high,komorowski2018artificial}) using estimators that leverage  importance sampling. Unfortunately, if some of the performance gains come from systematically avoiding actions taken in initial states with low performance, then it is likely that a similar performance benefit can also arise in the validation set if IS is used both in policy selection and later estimation. Even the estimator or objective involves a variance penalization (Eq.~\ref{eq:crm}), if only a small set of states are avoided, this may only mildly impact the variance and effective sample size, yet result in substantially overly optimistic estimates.

\textbf{Shift rewards to be strictly non-negative.} When a new policy assigns some contexts to actions not taken in the dataset, those tuples will contribute 0 to the vanilla IS objective. If the observed rewards for those contexts would always be negative, this yields to an overestimate. The benefit of avoiding such states disappears if all rewards are shifted to be non-negative and standard IS is used. However, vanilla importance sampling is well known to be high variance. Popular off-policy estimators like weighted IS are equivariant to any constant shift in rewards, and doubly robust estimators\cite{jiang2016doubly,thomas2016data} frequently center rewards around estimates of the reward/value outcomes. In both cases they can still suffer from the state context avoidance issues described above. 

\textbf{Estimated Behavior policy}. Prior work (**cite) has constrained the learned policy class to have overlap with the behavior policy, which is a minimal requirement for consistent estimation of a target policy using an importance-sampling based estimator. This can still cause the propensity overfitting problems described, when the dataset is insufficient to cover all non-zero behavior probability actions in all states, or when the behavior policy is itself unknown. An alternative is to estimate the behavior policy from data and use this both in the importance-sampling based objective, and to constrain the considered policy class to be ones with strict overlap with the estimated behavior policy. Indeed, semi-parametric theory (**check best ref) and past related work in bandits and RL (**cite Josiah, cite bandit AAAI paper) has suggested that even if the behavior policy is known, leveraging the estimated behavior policy can yield more accurate offline policy estimates, and it is natural to assume such benefits might also translate to improvements for constrained policy learning. While promising in principle, in large state space environments there are a number of subtle choices that lead to challenges to this approach. First, in such settings the maximum number of observed actions in any particular state is almost always one. Assuming there is good reason to believe that the behavior policy is not actually deterministic, it is necessary to use some function approximation method to estimate the behavior policy, such as work that has used linear or neural network approximations (**cite Xinkun, maybe Kallus?), or non-parametric methods like k-nearest-neighbors (**cite Ani). Unfortunately, as we will demonstrate in our experiments, we find that such approximators may be sufficient to sometimes accurately predict the behavior policy for a given state, but do not seem to provide as beneficial when used to constrain the targeted policy class. Such estimates may overestimate the probability of taking alternate actions in particular states, and therefore enable propensity overfitting by enabling policies that systematically avoid initial states leading to low reward, while still considering that such policies overlap with the estimated behavior policy. 


==> further_overfit.tex <==
We now highlight an important potential issue with using important sampling estimators during offline policy optimization. We first describe this for optimizing for contextual bandits using the self-normalized importance sampling estimator.

Let 
$v^\pi(x) = \mathbb{E}[r|x, a \sim \pi]$, $\hat{p}(x)$  be the empirical probability mass/density over the contexts $x$ in the dataset, and $W(x) = \sum_{i: x^{(i)} = x} \frac{W^{(i)}}{W}$ where $W$ is the importance weight (Equation~\ref{eqn:w}). We now decompose the importance weighted off-policy estimator into three parts. 
\begin{align}
    \hat{v} &= \underbrace{\mathbb{E}_{\hat{p}}[v^{\pi}(x)]}_{\text{empirical }v} + \underbrace{\sum_{x \in \Xcal} (\hat{p}(x)-W(x)) v^{\pi}(x)}_{\text{difference in context weights}}\\
    &+ \underbrace{\sum_{x \in \Xcal} W(x) \left( \sum_{x^{(i)}=x} \frac{W^{(i)}}{W(x)W} r^{(i)} - v^{\pi}(x) \right)}_{\text{weighted IS error in each context}}\notag
    \label{eqn:decomp}
\end{align}
The first term is a supervised empirical value estimate whose only error is due to the error in the empirical context distribution sampled in the dataset, vs the true context distribution. The second term captures the error caused by the difference between context distribution introduced by weights and empirical context distribution in the dataset. The third term computes the difference between the weighted IS estimate of the value of the policy in a specific context $x$ versus its true value $v^{\pi}(x)$, and then sums this over all contexts.

The second term is of particular interest, because it highlights how the IS estimator of a policy may effectively shift the relative weight on the context space. Note in the bandit setting (and in the initial starting state distribution for the RL setting) such shifting should not be allowed: the policy may control what actions are taken, but cannot change the initial  context distribution. 

%This decomposition shows that even each IS estimates of multi-arm bandit problem is accurate, the importance weighted objective can still be different from the supervised empirical value, caused by the improper distribution reweighing over the context.

Before illustrating the problematic behavior that can result from this type of objective function for offline policy learning, we first further analyze if it is possible for $W(x)$ to differ significantly from $hat{p}(x)$, given the normalization constraint of $\pi$. Expanding the difference between the empirical distribution over a context and $W(x)$: 
\begin{align}
    \hat{p}(x) - W(x) &= \hat{p}(x) - \sum_{i: x^{(i)} = x} \frac{W^{(i)}}{W}\\
    &= \hat{p}(x) - \frac{N*\hat{p}(x)}{W} \sum_{a} \hat{p}(a|x)\frac{\pi(a|x)}{\mu(a|x)} \\
    &= \left( 1 - \frac{N}{W} \right)\hat{p}(x)\\
    &\quad + \frac{N*\hat{p}(x)}{W} \sum_{a} \left(1-\frac{\hat{p}(a|x)}{\mu(a|x)}\right)\pi(a|x)\notag
\end{align}
While the first term is asymptotically zero because $W \to N$, the second term will be non-zero whenever the policy $\pi$ puts non-zero weight on actions in contexts where the empirical behavior distribution differs significantly from the true behavior distribution. Such a difference between the empirical and true behavior distributions can easily happen. This is especially the case in settings where the state-action space is large and the number of observed actions per state is small, which is common in recommendation settings, healthcare and many other applications. 

A policy learning algorithm maximizing the objective in Equation \ref{eqn:decomp} can exploit this difference in context weights and return a policy with an over inflated value  estimate, as we now illustrate: 

%The first term is asymptotically zero because $W \to N$.  However, the second term, when $\pi$ is optimized to maximize $v^\pi(x)$, can be far away from 0 when state-action space is large and the number of observed action per state is sparse. This overfitting problem exist in both self-normalized or vanilla importance weighting, one-step or multi-step problems, as we will show by two small examples.
\begin{example}
Consider a contextual bandit problem with $|\Xcal|$ contexts and $|\Acal|$ actions in each context. For half the  contexts $S_p$, the reward is $1$ for one action and zero for others. For the other half of the contexts, $S_n$, the reward is -1 for half the actions, and -5 for the rest. The true distribution over contexts is uniform. Note in this setting the optimal policy would have a reward of 0. The behavior dataset is draw from a uniform distribution over contexts and actions.  When the sample size $|\Dcal| < |\Acal|$, we can assume there is only one observed positive reward in the dataset. Then computing the policy to maximize the important sampling weighted objective will yield weights that are 0 on all contexts except for the context with the positive reward, through a policy $\pi$ that selects actions that are not present in the dataset for all contexts whose observed actions lead to only zero or negative rewards: let $\mathcal{A}_{s_i} = \{a_i :  r(s_i,a_i) \leq 0 \}$ then $\pi(s_i) = a_j$ where $a_j \notin \mathcal{A}_{s_i}$.

The resulting IS/SNIS estimator of the value of $\pi$ is $1$, which is much higher than the optimal policy value. In addition, note that the returned policy $\pi$ is likely to be worse  than the optimal policy for any context where  $r(s_i,a_i)=-1$, since that is the optimal reward possible for such states $s_i$, and by $\pi$ selecting an unobserved action $a_j$ in that state ($\pi(s_i)=a_j$), the policy $\pi$  may select an action with worse true reward,  $r(s_i,a_j)=-5$.
\end{example}

Note that in this example, there is no error in the importance weighted return for the contexts with positive $W(x)$ (which is the third term in the decomposition shown in Equation~\ref{eqn:decomp}). The issue arises because to optimize the objective, it is possible to select a policy whose $W(x)$ distribution over the contexts has zero weight on at least the half of the contexts with negative rewards $S_n$, by assigning them actions not selected in the dataset. This causes the second term in the decomposition (Equation~\ref{eqn:decomp}) to be significantly overestimated. 

%the third term in the decomposition shown in Equation~\ref{eqn:decomp} is zero However, in this example there is no guarantee that on all other contexts the learned policy select the rewarding action, except the observed action. We see that IS/SNIS significantly over-estimates the value. From the decomposition, the third term is zero -- importance weighted return in all MAB problems are accurate. The issue comes from the second term since the weights over context shift the true distribution, by "pretending" there is only one context. This examples shows the error in value estimates. With sequential settings or state aliasing, this can actually affect the policy selection as we will show next.

This is a unique overfitting phenomena in the  counterfactual (or called off-policy) learning settings since in supervised learning it is not possible for a  hypothesis $\pi$ to manipulate the weights over the input contexts. While this issue can arise in contextual bandits with large state and action space in small datasets, we show that it is even easier for this to occur in sequential reinforcement learning settings, even when only 2 actions are available in Example \ref{example:rl} and \ref{example:rl_model_fail} in the Appendix. 

Intuitively, the issue arises because in estimating the value of a new decision policy, it is acceptable to choose a policy that re-distributes the \emph{weights of actions within an initial context} but not re-distribute the \emph{weights across initial contexts}, since it is not a function of the actions selected. It is well known that in importance sampling, the expected ratio of the weights should be 1: $\EE_{y \sim \mu} [\pi(y)/\mu(y)] = 1$. In contextual policies, we expect that the expected weights should also be 1 for all initial contexts $x_0$: $\EE_{a \sim \mu(a|x_0)} \left[\pi(a|x_0)/\mu(a|x_0)|x_0\right] = 1$. 
% *EB: I'm still not sure this is said as clearly as I think we could-- could you take a pass please? 
However, optimizing for a standard importance sampling objective (such as Equation~\ref{eqn:decomp}) does not involve constraints that the empirical expectation of weights given an initial context $\empE\left[\ith{W_h}|\ith{x_h})|\ith{x_h}\right]$ (or the weights of $n$-step given initial context $\empE\left[\ith{W}|\ith{x_1})|\ith{x_1}\right]$ ) is still close to one. In order to optimize the future return, the optimization algorithm can optimize the weights of initial contexts in the dataset, instead of optimizing the weights on different actions/ action sequences in a given initial context. 

This result may seem surprizing, given that under mild assumptions which are satisfied here (Assumptions 1 and 2) importance sampling is well known to provide an unbiased estimate of the value of a policy. Our observations do not contradict this fact: while importance sampling will still provide an unbiased estimate given a policy, the policy optimization can exploit the finite sample error and its heterogeneousness across the policy class.
% how well their context-action distributions are represented in the available data, and policy optimization can exploit this. 

% discuss why previous work does not work



==> long_intro.tex <==
There has been a recent explosion in interest, from both the theoretical and algorithmic perspective, in offline/batch reinforcement learning. Offline RL is the study of how to leverage past existing datasets about sequences of decisions made, and their outcomes, in order to estimate the potential performance of potential automated decision policies or learn such automated decision policies. Studying this area offers numerous potential benefits, from allowing to potentially bring insights from RL to the growing number of application settings which produce such datasets (like healthcare~\citep{gottesman2019guidelines,nie2021learning}, customer marketing~\citep{bottou2013counterfactual,thomas2017predictive} or home automation~\citep{emmons2022the}), to potentially providing ways to leverage vast amounts of observational training data encoded in videos~\citep{chang2020semantic,pmlr-v155-schmeckpeper21a}% (consider youtube as a training data set for training robots to cook, folder laundry or entertain at parties)
, to advancing our core understanding of the data characteristics needed to learn near optimal policies. 

One of the most exciting possibilities is that offline RL could be used to leverage existing variability in past decisions to uncover better decision policies for future use for scenarios where there are many barriers or challenges to performing explicit experimentation or online RL, such as healthcare, education or autonomous driving. However, such settings offer important differences than much of the focus in offline reinforcement learning: the domain may not be Markov in the available feature set and knowledge of the behavior decision policy is typically unknown. This has inspired work on offline policy evaluation estimation methods that make minimal assumptions on the data generation process, such as importance sampling and doubly robust estimation methods~\citep{precup2000eligibility,Jiang2016} which have also formed the backbone of offline policy learning methods that leverage such estimators as part of their policy search approach~\citep{huang2020importance,cheng2020trajectory}.

Unfortunately, we show that offline policy selection or learning algorithms that rely on such offline estimation methods that leverage importance sampling can suffer from a key flaw that we denote as \textit{propensity overfitting}. In brief, the structure of the policy estimator is such that high estimated performance can be achieved both by policies that have high average performance, and by policies that systematically avoid taking actions taken in the dataset for initial states that lead to low rewards. This can substantially inflate the estimated performance of a potential decision policy when there may be some states for which any decision policy will result in lower rewards than some other states. As an intuition, consider a setting where some patients arrive much sicker than some healthier patients. In this setting, any policy for the sicker patients will likely yield slightly worse outcomes than the average outcomes for healthier patients, but a policy’s value must be taken in expectation over all patients, not just the healthy patients. We detail how a number of methods, including those that have been proposed before for other reasons, do not solve this issue, including: using a validation set, shifting the reward baseline, and leveraging thresholds on an estimated behavior policy. 
[**cite david? Did they just discuss for bandits?] % yes it's only for bandits


Fortunately, we show that a relatively simple method for constraining the policy class considered with off policy learning can greatly ameliorate the problem of propensity overfitting. Our approach can be viewed as related to pessimistic offline RL in Markov decision processes, which has roots at least since the early 2000s in the robust MDP literature (**cite drew, Berkeley people, marek? Etc], was revived recently~\citep{DBLP:conf/uai/LiuSAB19,satija2021multiobjective} and has been receiving growing attention with a number of significant empirical improvements (** cite a bunch) and theoretical advances (**cite) in continuous state and/or action settings and in conjunction with deep RL. One of the key tenants of pessimistic offline RL, which is similar to many advances in optimistic online RL (**cite), is to maintain precise quantification over the uncertainty over  the model parameters and/or value functions of the Markov decision process, given the available data. Doing so when the state and action space is finite is well understood: it is sufficient to maintain counts of the number of observations of each  (state,action) or (state,action, next state) tuple, in order to compute precise confidence bounds over the resulting model parameters or resulting value function. However, a  key challenge is how to quantify statistical uncertainty when the state space is extremely large or continuous, and this issue is perhaps even more paramount in offline RL settings where we wish to leverage importance-sampling based estimators in order to make minimal assumptions over the data generation process. We show here that constraining the policy class per state only to actions taken in the data for nearby states, which may be viewed as a loose analogy to count based uncertainty, is sufficient to lower bound the amount of propensity overfitting that can occur. Our approach still ensures asymptotic consistency of the estimation of any policy covered by the behavior policy\footnote{Coverage is a minimal requirement for all IS methods to be consistent estimators of a new proposed policy.} while providing significant benefits in the finite regime, by essentially regularizing the policy back to the behavior policy when there is insufficient data. In this way, our method is related to other methods that revert back to the behavior policy given minimal data for MDP model or value function learning~\citep{satija2021multiobjective} or in the bandit setting~\citep{sachdeva2020off,brandfonbrener2020offline}. To our knowledge our work is this first to explore this for general stochastic decision processes or policy search methods, and also the first to consider how to do this when the behavior policy is unknown or when the state and action space is sufficiently large that careful attention to being precise about what it means for a state-action pair to be sufficiently well estimated is paramount. [**revise this to be precise. Spibb did look at large spaces but not sure thought about how to regularize back to $pi_b$ in such spaces and if $pi_b$ is unknown]. 

We show in simulations and in a real dataset on patient sepsis outcomes that our approach learns policies with significantly higher expected rewards than prior methods, and that those estimates are expected to be reliable, with solid effective samples sizes. Our results highlight and remediate a potential reliability barrier for offline RL with minimal data process and realizability assumptions, and suggest interesting open issues about the role of quantifying uncertainty in offline datasets. 



==> old_experiment.tex <==
To illustrate the benefit of avoiding overfitting importance weights, w

We now compare \ispg with several prior works in offline RL. The most relevant work in avoiding overfitting when using importance sampling is norm-POEM\cite{swaminathan2015self}, that uses a  counterfactual risk minimization objective function for offline contextual bandits. Here 

and exponential family of distributions to model $\pi$: while designed for contextual bandit settings, 
Here we extend it here to be suitable for sequential decision settings and use a neural network policy class: . We compare with a baseline algorithm using norm-POEM and neural networks function approximators and refer to it as \ispgbaseline in this section. Constraining the action by thresholding $\mu(a|s)$ is used in prior work as a trick the stabilizing the objective \citep{futoma2020popcorn}, and is also included in the comparison referred as \ispgknn. We also compared with recent deep value-based method in batch RL: BCQ \citep{fujimoto2019off} and PQL \citep{liu2020provably}. For all these algorithms including ours, we use a feedforward neural network as function approximators.

In both two experiments below, we follow the same procedures for all algorithms to select their hyper-parameters. All algorithms are trained on the training set with all hyper-parameters and several restarts, saving checkpoints during the training, then we select the checkpoint with the highest self-normalized truncated IS (SNTIS) estimates on a hold-out validation set. Finally, we report the test performance of selected policy. In the simulation experiment, it is measured by the online Monte-Carlo estimates and in the real dataset experiment, is measured by SNTIS estimates on the test set. The experiment details including steps between checkpoints, hyper-parameters range, and the number of re-start are in Appendix. 
% details: sample size, checkpoints, hyperparameters, random seeds

\subsection{Experiment in LGG Tumor Growth Inhibition Simulator}
We first test different policy optimization in a previously proposed Tumor Growth Inhibition (TGI) simulator \citep{ribba2012tumor} to verify the effect on overfitting. The simulator describes low-grade gliomas (LGG) growth kinetics in response to chemotherapy in a horizon of 30 steps (months), with an non-Markov context space, binary action space of drug dosage \citep{yauney2018reinforcement}. The reward at each step consist of an immediate penalty proportional to the drug concentration, and a delayed reward of the decrease in mean tumor diameter. The behavior policy is a fixed dosing schedule of 9 months (the median duration from \cite{peyre2010prolonged}) plus $30\%$ of a uniformly random choice of actions. The training and validation set both have 1000 episodes.

In this experiment, the behavior policy can only take values in $\{0.15, 0.85\}$ so there is only one non-trivial thresholding on $\mu(a|s)$ in the baseline \ispgknn, which results in a fixed policy as the deterministic part of behavior policy, included as $9$-mon in Table \ref{tab:tumor_result}. We repeat the experiment 5 times with 5 different train and validation sets to report the mean and SEM of metrics in Table \ref{tab:tumor_result}. Policy values are normalized between $0$ (uniform random) and $100$ (best policy from online RL). It shows \ispg achieves the highest test value as well as a smaller variability compared with others. 

\textbf{Does \ispg reduce overfitting?} We calculate the difference between $\wtis$ on validation set and the online test value. Though it is off-policy evaluation on the validation set, most algorithms still have a significant overestimates, which reflect the overfitting particularly due to the off-policyness and is different from the standard loss overfitting in supervised learning. 

\textbf{Performance comparison in MDP environment} We also repeat the experiment with an MDP modification of the simulator, including an immediate Markovian reward and additional features for a Markovian state space. Compared with Q learning approaches relying on Markov assumptions, our algorithm is only slightly worse, and still largely outperform the policy-based approaches.

% \textbf{Is the learned policy medically reasonable?} We also reported the amount of drug dosing (number of months with full dose) and the percentage of change in MTD. Compared with a fixed dosing of 9 month with MTD decrease $49.84\%$, our algorithm decrease MTD by $-38.04\%$ with only $5.49$ months of using drug. Other RL algorithm take less drug dosing but have a significant disadvantage in the MTD decrease.

\begin{table*}[t]
    \centering
    \begin{small}
    \begin{tabular}{c|c|ccccc}
        \toprule 
         & Algorithms & \ispg & \ispgbaseline & BCQ & PQL & $9$-mon \\
         \midrule 
         Non-MDP & Test $v^\pi$ & $ 92.20 \pm 1.63 $ & $75.06 \pm 13.22$ & $30.24 \pm 15.22$ & $74.76 \pm 9.75$ & $68.12 $ \\
         & $\wtis - v^\pi$ & $ -1.26 \pm 1.92$ & $15.57 \pm 13.07$ & $63.72 \pm 15.54$ & $17.74 \pm 9.49$ & $-$ \\
        %  Drug dosing & $5.31 \pm 0.31 $ & $3.81 \pm 1.00$ & $\textbf{0.80} \pm 0.72$ & $2.56 \pm 0.56$ & $9$ \\
        \midrule
        MDP & Test $v^\pi$ & $89.52 \pm 1.55$ & $78.79 \pm 6.42$ & $95.64 \pm 4.64 $ & $96.88 \pm 3.76$ & $68.12$ \\
        & $\wtis - v^\pi$ & $ 5.16 \pm 1.78$ & $14.93 \pm 5.71$ & $-0.69 \pm 0.81$ & $0.55 \pm 5.12$ & $-$ \\
         \bottomrule
    \end{tabular}
    \end{small}
    \caption{Test $v^\pi$ and amount of overfitting of the learned policy. Test $v^\pi$ is computed from 1000 rollouts in the simulator. $\wtis$ on the validation set $-$ test $v^\pi$ represents the amount of overfitting. %Drug dosing and treatment effect measured by MTD change is computed from the test rollouts. 
    All numbers are averaged across 5 runs with the standard error reported.}
    \label{tab:tumor_result}
    \vspace{-0.3cm}
\end{table*}

\subsection{Experiment in ICU data - MIMIC III}
We demonstrate our method in a real-world example of learning policies for sepsis treatment in medical intensive care units (ICU). We use an extracted cohort \citep{komorowski2018artificial} of patients fulfilling the sepsis-3 criteria from the MIMIC III data set \citep{johnson2016mimic}\footnote{ The dataset is available upon application and training: https://mimic.mit.edu/iii/gettingstarted/. The code to extract the cohort is available on: https://gitlab.doc.ic.ac.uk/AIClinician/AIClinician.}. This cohort consists of data for 14971 patients. The contexts for each patient consist of 44 features, 
%including demographics, Elixhauser premorbid status, vital signs, laboratory values,
summarized in 4-hour intervals, for at most 20 steps. The actions we consider are the prescription of IV fluids and vasopressors. Each of the two treatments is binned into 5 discrete actions according to the dosage amounts, resulting in 25 possible actions. The rewards are defined from the 90-day mortality in the logs, $100$ if survived and $0$ otherwise. 

In this experiment, as we have no simulator to test the learned policy, we hold out $20\%$ of data for validation and $20\%$ of data for the final test. Since the treatment logs do not include the probabilities of actions, we estimated the probabilities of clinicians' policy by $k$-NN with $k=100$ which is used in a previous study of this dataset \citep{raghu2018behaviour}. As $\hat{\mu}(a|s)$ is no longer always positive, for all policy optimization algorithms we requires $\pi(a|s) > 0$ only if $\hat{\mu}(a|s) > 0$. 
Since the test is done through off-policy evaluation (SNTIS), test results decided by only a very small number of samples and are unreliable, which is measured quantitatively by the effective sample size (ESS) \citep{owen2013monte}. To make sure the test effective sample size is large and evaluation is reliable, we select policies on the validation set with effective sample size is no less than $200$. 

In Table \ref{tab:sepsis_result}, we report SNTIS estimates of selected policy on the test set and calculate the $95\%$ upper and lower bound from bias-corrected and accelerated (BCa) bootstrap. Clinician's policy value is the averaged reward on the test dataset, confidence bounds are computed from BCa bootstrap in the same way, and ESS of the clinician's policy is the sample size. The results show that \ispg achieves not only the highest evaluation on the test set but also a higher effective sample size compared with other methods. With the highly non-Markov context space, policy optimization methods perform better than value-based batch RL algorithms. 

\begin{table*}[t]
    \centering
    \begin{small}
    \begin{tabular}{c|ccccc|c}
        \toprule 
         Method & \ispg& \ispgknn & \ispgbaseline & BCQ  & PQL & Clinician \\
         \midrule 
        Test SNTIS & 91.46 (90.82) & 87.95 & 87.71 & 82.67 & 84.40 & 81.10 \\
        $95\%$ BCa UB & 93.24 (92.61) &	90.58 &		90.04 & 86.83 &	88.29 & 82.19 \\
        $95\%$ BCa LB & 89.59 (88.68) & 84.77 &	84.90 & 78.25	& 80.13 & 79.80\\
        Test ESS & 624.92 (586.37) & 372.00 & 399.59 & 228.82 & 231.93 & 2995 \\
         \bottomrule
    \end{tabular}
    \end{small}
    \caption{Test evaluation, $(0.05, 0.95)$ BCa bootstrap interval, and effective sample size in the sepsis cohort of MIMIC III dataset. Value inside parenthesis of \ispg is without CRM variance penalty. }
    \label{tab:sepsis_result}
    \vspace{-0.3cm}
\end{table*}

\textbf{Is the variance regularization helpful?} To demonstrate the effect of variance penalty on the \ispg algorithm, we demonstrate the test performance \ispg without the variance penalty. The performance is worse than using the variance penalty but still higher than baseline algorithms.

\textbf{The trade-off between effective sample size and performance estimates} Among the evaluation of different policies from the same algorithm on the validation set, we observe a trade-off between the effective sample size and self-normalized truncated IS estimates. Some hyper-parameters are more restricted to the behavior policy resulting in high ESS but lower estimates, and some vice-versa. In Figure \ref{fig:sepsis_tradeoff} we plot each hyper-parameter and each re-start from different algorithms on the ESS-SNTIS plain. The plots show that \ispg achieves a better Pareto frontier between performance estimates and effective sample size than other algorithms.

\textbf{Do learned policies take medically reasonable actions on high-stake patients?}
% Preliminary study about off-policy evaluation in healthcare problems \citep{gottesman2019guidelines, gottesman2018evaluating} highlight that it is also important to diagnose the interpret the learned policy given the high variance in statistical method. 
One key phenomenon of the overfitting issue is avoiding contexts with low expected rewards to achieve good IS/SNIS score. So we are interested in for those patients with severe conditions, whether the learned policy gives simply avoids the logged actions or medically reasonable choice. We select the logs with a high SOFA score (measuring organ failure) in the test dataset. Figure \ref{fig:sepsis_highsofa_visualization} depicts the number of actions taken by different policies as well as the clinicians on the high-SOFA contexts. \ispg mainly takes high-vasopressors high-IV-fluid treatments but also some IV-fluid-only treatments, which is similar to the clinician's policy but more concentrating on high-vasopressors treatments. \ispgbaseline and value-based methods, take treatments that are different from the logged policy, indicating that the learned policy might try to avoid the contexts with high SOFA in the distribution.

\begin{figure*}[t]%{R}{0.8\textwidth}
    \begin{minipage}{0.4\textwidth}
    \centering
    \includegraphics[width=0.9\textwidth]{mimic_ess_tradeoff.png}
    \subcaption{Trade-off between ESS and OPE}
    \label{fig:sepsis_tradeoff}
    \end{minipage}
    \begin{minipage}{0.56\textwidth}
    \centering
    \includegraphics[width=0.9\textwidth]{highsofa_main.png}
    \subcaption{Action counts in high-SOFA contexts}
    \label{fig:sepsis_highsofa_visualization}
    \end{minipage} 
    \caption{(a): Trade-off between effective sample size and value estimates. (b): Action counts heatmap in high-SOFA contexts of the policy learned.}
    \vspace{-0.3cm}
\end{figure*}


==> old_intro_pre_uai2022_submission.tex <==
% In previous chapters, we discussed batch policy learning algorithms with either actor-critic or $Q$ learning algorithm. In this chapter, we study batch reinforcement learning in a non-Markov environment. In this case, the value function and model-based approach are more vulnerable to the unknown error of mis-specified models. 

Learning decision policies from offline data has a critical impact on real-world decision-making applications such as healthcare \citep{lei2012smart,komorowski2018artificial}, recommendation systems \citep{li2010contextual,chen2019top}, and intelligent tutoring systems \citep{mandel2014offline}.%, and received a surge of attention recently as batch reinforcement learning (RL) \citep{levine2020offline,fujimoto2019off,kumar2019stabilizing,liu2020provably,kumar2020conservative,yu2020mopo,kidambi2020morel} and batch contextual bandit\citep{sachdeva2020off,kuzborskij2021confident,karampatziakis2021off}. 
 In real-world decision-making applications, we often need to use limited amounts of data about past decisions to yield better future performance in complex, hard-to-model domains. Such offline policy optimization encounters two key generalization challenges:  distribution shift and modeling bias. 
 Distribution shift arises because, under a new decision policy, the distribution of observations and actions will be different than the distribution of observations and actions in the offline data. 
 %means the distribution of outcome including future observations we observe in the dataset will be different from the true distribution if we execute the hypothesis policy online -- In offline settings, we have no new observations. 
 Modeling bias can occur when popular assumptions over the domain structure or model class (such as the Markov assumption, realizability, or the value function class being closed under the Bellman), fail to hold in the problem setting. Learning from limited data, algorithms ignoring these challenges can produce policies and estimates of policy performance that are far more optimistic than they achieve in practice, similar to the overfitting in supervised learning.

To address this, prior work in batch reinforcement learning (RL) and contextual bandits mostly falls into two categories: (1) changing the estimator or loss function used in computing offline value estimates, or (2) constraining the policy search space. In category (1),  self-normalized IS (or weighted IS)  \citep{hesterberg1995weighted,swaminathan2015self}, variance regularization \citep{swaminathan2015counterfactual,metelli2018policy}, doubly robust methods\citep{dudik2011doubly,jiang2016doubly,thomas2016data}, and  uncertainty regularized model-based batch RL \citep{yu2020mopo,kidambi2020morel} are all approaches that aim to provide more stable and variance-penalized estimates of a policy's performance to address the uncertainty due to limited data and distribution shift. The second category of direct constraints on the policy class includes bandit learning under action/policy constraints with behavior probability \citep{sachdeva2020off}, value-based batch RL algorithms by constraining the policy disagreement \citep{kumar2019stabilizing,buckman2020importance}, thresholding the action probability \citep{fujimoto2019off,futoma2020popcorn}, or thresholding the marginalized state-action probability \citep{liu2020provably}, under the behavior policy.

Many of the works above rely on learning MDP models or value functions based on MDP assumptions. However, the Markov assumption and function approximation assumptions are often unrealistic in real-world problems and hard to verify, which limits their eligibility in certain application problems. In this paper, we consider learning an policy to optimize an importance weighted return, as it is free from Markov and other types of model assumptions. We identify an unique overfitting that is not solved in prior work about policy optimization and propose a new constraint on policy named \emph{eligible actions} (EA) to address the overfitting issue.

The overfitting issue comes from fitting the importance weights in the weighted return objective. The importance weighted return can effectively remove a certain subgroup of samples in the dataset by decreasing all weights to zero. This context avoidance is unrealistic when the subgroup consists of a subset of initial states, as the policy does not get to control the initial state distribution. 
Consider the following motivating example: an AI decision policy may learn from historical treatment logs to avoid all the logged treatment in the history for patients with severe conditions as they lead to low rewards. This avoidance can be achieved with finite data if the action space is large, and such avoidance will result in high off-policy estimates. However, in the real environment, a policy still should make good decisions for patients who arrive with severe conditions. This \emph{propensity overfitting}  problem was studied in contextual bandit problems \citep{swaminathan2015self}. While their solution effectively constrained the upper bound on importance weights on high-reward samples, the challenge of overfitting to avoid the low-reward samples remains. % Our solution is based on an key observation that the the policy should optimize the weights of roll-out actions/states but not the sum of weights in all initial/roll-in states. We observe that the policy optimization should affect the weights of actions and outcome by choosing probabilities on actions. However, it should not optimize the sum/expectation of weights on a state that is correlated to the following actions, because the prior state is controlled by the actions. For policy evaluation, when policy is independent from the data this is not an issue as the expectation of importance weights given a state is 1. However, when optimizing the policy on data, the policy can manipulate the state distribution through fitting the weights on later actions, and the empirical mean of weights on a state will be away from its expectation $1$ which causes the overfitting in weighted return. 

\textbf{Our contribution} 
To address the issue that optimizing with propensity weights may avoid certain initial states, we propose the \textbf{P}olicy \textbf{O}ptimization with \textbf{EL}igible \textbf{A}ctions (\ispg) algorithm. %Similar in spirit to recent Markov methods (e.g.\cite{liu2020off}), 
We constrain the potential action set to the set of observed actions with similar states to prevent improper avoidance to lower-reward initial states. Thus within a radius of a particular state, the sum of observed importance weights are always lower bounded. We then study the empirical performance of \ispg in a medical simulator and a real-world medical dataset. %compared with prior work against importance weights overfitting and SOTA value-based batch reinforcement learning algorithms. 
Our approach finds much better decision policies than prior state-of-the-art algorithms in both domains.  % performance against the importance weights overfitting and achieves higher evaluation value.


==> old_prior_work.tex <==
Before we describe a method to alleviate this problem, we first review prior work. %The overfitting issue in batch policy optimization comes from finite-sample overly optimistic estimates of policies, which can cause suboptimal policies to be selected, and has been discussed as
There is increasing interest in multi-armed bandits and offline RL to avoiding overly optimistic estimates of policies computed from finite datasets that can cause suboptimal policy learning, and prior work has discussed 
extrapolation error\citep{fujimoto2019off}, propensity overfitting \citep{swaminathan2015self}, and bandit error \citep{brandfonbrener2020offline}. The problem we identified arises specifically from deficient support in the observed dataset. 


To address potential overfitting, one line of work focuses on changing the objective used for policy optimization. For example, \citet{swaminathan2015self} has shown that policy optimization using vanilla importance sampling in contextual bandits will over-maximize the weights if the reward is positive and over-minimize the weights for negative reward. Shifting the rewards will help with the latter (and avoid part of the context avoidance we describe) but can worsen the former. The self-normalized estimator proposed to address the issue of over-maximizing reward~\citep{swaminathan2015self} is  equivariant to any constant shift in rewards, and will still suffer from the context avoidance issues we describe above. Counterfactual risk minimization~\citep{swaminathan2015counterfactual} uses variance regularization based on the empirical Bernstein's inequality. 
% Prior work in contextual bandits\citep{swaminathan2015counterfactual,swaminathan2015self} included a variance penalization . This can be naturally extended to the multi-step setting to yield a target objective for offline policy learning: 
However, this penalization is at the policy level and does not directly address the problem with avoiding contexts with low reward. In Appendix Figure \ref{fig:overfitting_example_result} we show the counterfactual risk minimization regularization with or without self-normalization requires a  large dataset to perform well. Later work \citep{joachims2018deep} extended norm-POEM to stochastic gradient descent settings for large-scale training. 
Recent work \citep{brandfonbrener2020offline} discussed a similar overfitting issue as we describe and compared the performance of offline policy optimization and model/value-based method on this overfitting issue. Those authors focus primarily on the negative result of the policy optimization approach and the advantage of the model/value-based method. Doubly robust estimators \citep{dudik2011doubly,jiang2016doubly,thomas2016data,kallus2019double,kallus2019efficiently} have multiple benefits but as long as the learned $Q$ function is imperfect, policy learning can still overfit to the high/positive residual $r - Q$. Pessimism under uncertainty approaches are promising ~\citep{kidambi2020morel,yu2020mopo} but have so far only been developed for Markov settings and are not robust to model class misspecification.




Another line of offline batch policy optimization constrains the policy search space, for example to constrain target policies to be close in some distance to the behavior policy~\citep{kumar2019stabilizing,buckman2020importance}. A common approach is to constrain target policies to have a minimum  conditional action probability under the behavior policy $\mu(a|s)$ (e.g. \citet{ sachdeva2020off,fujimoto2019off,futoma2020popcorn,liu2020provably}). This work has focused on algorithms and analysis for the Markov setting with additional model realizability assumptions, except ~\citet{sachdeva2020off} in the bandit case and ~\citet{futoma2020popcorn} in the RL setting. For example, the MDP value based approaches often require the value function class is closed respect to the Bellman operator and the value function is realizable. Such assumptions are hard to verify in real-world domains. %Empirically, the ``deadly-triad'' \citep{sutton2018reinforcement} describes the instability when combining the off-policy learning with self-bootstrap. 

%These directions are promising, particularly in situations where the behavior policy has deficient support and policy optimization should be constrained to policies with sufficient overlap. However, they
This prior work does not address the issues we outlined, that occur due to deficient support in the observed finite data rather than in the expected behaviors. %More precisely, recall in our motivating examples $\mu(a|s)$ is uniform thus it provides little information on which actions lead to larger overfitting risk. Instead the overfitting is caused by taking actions avoid the logged data purposely, instead of taking action to avoid the low conditional probability $\mu(a|s)$. 
Our work can be broadly viewed as following in the recent line of work on pessimism under uncertainty, but adapted to provide policy search based offline learning method that does not require the Markov assumption or model realizability assumptions, and can achieve strong performance given a finite dataset.


% The setting does not satisfy the Markov assumption and so the value function or MDP model based approaches also fail in this setting. 
% This overfitting problem is related to the \emph{propensity overfitting} issue discussed in previous literature in contextual bandit settings. Over-weighing the weights for high-rewards contexts, as well as over-avoiding the weights for low-rewards contexts are the two sides of the same propensity (importance weights) overfitting issue: fitting the weights of context instead of the weights of actions. The norm-POEM \citep{swaminathan2015self} method use self-normalized IS estimator to avoid over-weighing high reward boundlessly. The self-normalization of weights cannot prevent over-avoiding the low-rewards contexts, which eventually also result in over-weighing high reward in a self-normalized estimator. CRM's variance penalty \citep{swaminathan2015counterfactual} method relieves the overfitting problem by the variance penalization. It combats both the unavoidable variance from reward/transition dynamics and the variance from importance weights, thus might fail to avoid the overfitting in importance weights when the variance from the environment is non-uniform. 

==> original_overfitting.tex <==
{\color{red}
Optimizing such an objective can be viewed as a supervised learning problem with a loss function $-\ith{r_h} \ith{W}$, where $\pi$ intend to optimize the loss $-\ith{r} \ith{W}$ by maximizing the $\ith{W}$ for actions with positive $\ith{r}$ and minimizing $\ith{W}$ for actions with negative $\ith{r}$. However, such a process raises up a unique overfitting problem due to the weights $\ith{W}$ can also improperly change the importance of context $\ith{x}$. %\footnote{Notice that with proper choice of control variate to minimize variance -- either additive or multiplicative (self-normalized IS) -- $\ith{r}$ will be centered around zero.}
We first illustrate this by a decomposition of the one-step importance weighted learning objective. Similar decomposition can also be established and explain the overfitting problem in multi-step as shown in the appendix. Define $v^\pi(x) = \mathbb{E}[r|x, a \sim \pi]$, $\hat{p}(x)$ to be the empirical probability mass/density over $x$ in the dataset, and $W(x) = \sum_{i: x^{(i)} = x} \frac{W^{(i)}}{W}$. We can decompose the importance weighted off-policy estimator into three parts.
\begin{align}
    \wtis &= \underbrace{\sum_{x \in \Xcal} \hat{p}(x) v^{\pi}(x)}_{\text{empirical }v} + \underbrace{\sum_{x \in \Xcal} (\hat{p}(x)-W(x)) v^{\pi}(x)}_{\text{difference in context weights}} + \underbrace{\sum_{x \in \Xcal} W(x) \left( \sum_{x^{(i)}=x} \frac{W^{(i)}}{W(x)W} r^{(i)} - v^{\pi}(x) \right)}_{\text{weighted IS error in each context}}
\end{align}
The first term is a supervised empirical value estimates, which is the best estimator we can hope to achieve in the off-policy setting. The second term demonstrated the error caused by the difference between context distribution introduced by weights and empirical context distribution in the dataset. The third term, is the weighted sum of importance sampling errors in multi-arm bandit problems of each context. This decomposition shows that even each IS estimates of multi-arm bandit problem is accurate, the importance weighted objective can still be different from the supervised empirical value, caused by the improper distribution reweighing over the context.

We may ask that, is it really possible that $W(x)$ is far from $\hat{p}(x)$ given that $W(x)$ must satisfy the normalization constraint of $\pi$. We further breakdown this term.
\begin{align}
    \hat{p}(x) - W(x) &= \hat{p}(x) - \sum_{i: x^{(i)} = x} \frac{W^{(i)}}{W} = \hat{p}(x) - \frac{N*\hat{p}(x)}{W} \sum_{a} \hat{p}(a|x)\frac{\pi(a|x)}{\mu(a|x)} \\
    &= \left( 1 - \frac{N}{W} \right)\hat{p}(x) + \frac{N*\hat{p}(x)}{W} \sum_{a} \left(1-\frac{\hat{p}(a|x)}{\mu(a|x)}\right)\pi(a|x)
\end{align}
Though the first term is asymptotically zero, the second term, when $\pi$ is optimized to maximize $v^\pi(x)$, can be far away from 0 when state-action space is large and the number of observed action per state is sparse. This overfitting problem exist in both self-normalized or vanilla importance weighting, one-step or multi-step problems, as we will show by two small examples.
\begin{example}
Consider a contextual bandit problem with $|\Xcal|$ contexts and $A$ actions in each context. For all contexts, the reward is $1$ for only one action and zero for others. The dataset is draw from a uniform distribution over contexts and actions. When the sample size $|\Dcal| < A, |\Xcal|$, we can assume there is only one observed positive reward in the dataset. Thus, IS/SNIS will fit the weights such that it is $1/A$ for that observation and zeros for all others. Thus SNIS estimates is $1$.
\end{example}
However, in this example there is no guarantee that on all other contexts the learned policy select the rewarding action, except the observed action. We see that IS/SNIS significantly over-estimates the value. From the decomposition, the third term is zero -- importance weighted return in all MAB problems are accurate. The issue comes from the second term since the weights over context shift the true distribution, by "pretending" there is only one context. This examples shows the error in value estimates. With sequential settings or state aliasing, this can actually affect the policy selection as we will show next.

\begin{example}
Consider a sequential treatment problem as shown in Figure \ref{fig:overfitting_example}. We need to make the decision between two actions in the first step. Both actions have a positive treatment effect on half of the patients leading to $r=1$. Action 1 has a side effect ($r=-1$) on the other half of the patients. Action 2 has a stronger side effect ($r=-5$) on the other half of the patients, however, not immediately observed. These patients will be treated with $H-1$ more steps with $A$ actions, leading to $A^{H-1}$ different action sequences. In this example, data are draw from an uniform random policy $\mu(a=0|x_1) = \mu(a=1|x_1)$ = 0.5, and the probability of each action sequence following $a=2$ is $\frac{1}{A^{H-1}}$. When $A$ and $H$ are large, there always exists a sequence that is not observed in the dataset. In this case, the policy taking action 2 at the first step and the unseen path in the following steps will be overestimated significantly by IS or self-normalized IS. Thus the offline policy optimization will prefer taking action 2 at the first step as a result of overfitting. 
\end{example}
}

  

\begin{figure*}[th]%{R}{0.8\textwidth}
%\vspace{-\intextsep}
%\hspace*{0.5cm}
    \begin{minipage}{0.45\textwidth}
    \centering
    \includegraphics[width=0.8\textwidth]{example_patient.pdf}
    \subcaption{Example of overfitting importance weights}
    \label{fig:overfitting_example}
    \end{minipage}
    \hspace{0.5cm}
    \begin{minipage}{0.45\textwidth}
    \centering
    \includegraphics[width=0.8\textwidth]{toy_example_result.png}
    \subcaption{Number of samples to solve the example for $A=2$ and different $H$.}
    \label{fig:overfitting_example_result}
    \end{minipage}
\end{figure*}

Again we see the policy tries to avoid the logged actions on the sick patients, such that these patients contribute no weights in the weighted return policy evaluation. However, as a result of the previous action, these sick patients are not avoidable in the true environment. Thus this way of optimizing the weights is an overfitting in the offline dataset. This is a unique overfitting in counterfactual (or called off-policy) learning settings since in supervised learning there is no way for the hypothesis $\pi$ to manipulate the weights over input context.

How could that happen as we know importance sampling estimator provides a valid estimation of the counterfactual outcome? The IS estimator re-weight the actions but not re-weight the distribution of context as these are not affected by the following-up actions. This is confirmed by the per-context normalization condition that $\EE\left[\pi(a|x)/\mu(a|x)|x\right] = 1$. That means, when we optimize the importance weighted return, we wish to re-distribute the \emph{weights of actions within a context} but not re-distribute the \emph{weights across contexts}. However, when we optimize the policy on a dataset $\Dcal$, we have no constraints on that the empirical expectation of weights given the context $\empE\left[\ith{W_h}|\ith{x_h})|\ith{x_h}\right]$ (or the weights of $n$-step given initial context $\empE\left[\ith{W}|\ith{x_1})|\ith{x_1}\right]$ ) is still close to one. In fact, with a large policy class $\Pi$, it is possible and, in fact, very common, to maximize the weighted return by re-distribute the weights across context. For low-rewards (initial) context, the policy tends to avoid all logged actions so the weights given the context are always zero, and vice versa for high-reward contexts. This observation provides us an interpretation of overfitting: In order to optimize the future return due to roll-out actions in certain context, the optimization algorithm optimizes the weights of roll-in or initial contexts in the dataset, instead of optimizing the weights on different roll-out actions sequences in one context. 

% discuss why previous work does not work

\paragraph{Prior work on overfitting in offline policy optimization} Before we start our solution to this problem, we first review how the overfitting/estimation error issue is generally addressed in previous batch RL and contextual bandit settings. Then we discuss why existing approaches does not fully address the overfitting issue of importance weights here. 

In general, the overfitting issue in batch policy optimization appears as the estimates of policies that are far more optimistic than they achieve in practice. This is related what was summarized as extrapolation error\citep{fujimoto2019off}, the propensity overfitting \citep{swaminathan2015self}, bandit error \citep{brandfonbrener2020offline}. Though some of them cover the overall overfitting in off-policy objective, and some focus more specifically on the importance weights. To address this prior work mostly falls into two categories: One way of doing that is change the estimator used to evaluate the target policy as the objective of policy optimization. The other is to constrain the policy class to limit the policy optimization on those policy with less overfitting. 

With in the first category, a natural question to ask is whether we can avoid the overfitting by shifting the reward, for example, to be always positive in the example above. As discussed in \citep{swaminathan2015self}, with vanilla importance sampling estimator, policy optimization will over-maximize the weights if the reward is positive and over-minimize the weights for negative reward, such that the weighted return can exceed the valid range. This is summarized as the propensity overfitting in \citep{swaminathan2015self}, and it propose self-normalized estimator to address the issue, which is equivariant to any constant shift in rewards. With self-normalized estimator,  Over-weighing the weights for high-rewards contexts, as well as over-avoiding the weights for low-rewards contexts are the two sides of the same importance weights (propensity) overfitting issue, as the weights will be normalized according to the sum of weights in all samples. Self-normalization can avoid over-weighing high reward boundlessly, but cannot prevent over-avoiding the low-rewards contexts, which also cause propensity overfitting issue as we discussed in the motivating example. Another orthogonal change of objective function in prior work \citep{swaminathan2015counterfactual} is counterfactual risk minimization method using variance regularization. It combats both the unavoidable variance from reward/transition dynamics and the variance from importance weights, thus might fail to avoid the overfitting in importance weights when the variance from the environment is non-uniform. Doubly robust estimators \citep{dudik2011doubly,jiang2016doubly,thomas2016data} is a common way against the variance in importance weights. However as long as the learned $Q$ function in the doubly robust estimator is imperfect, the residual $r - Q$ still varies then the importance weights can still overfit to the high/positive residual context. In multi-step settings, the efficient control variate is the $Q$ function \citep{kallus2019double,kallus2019efficiently} and thus it requires the same assumptions as the value-based approach. Some model-based batch RL algorithms \citep{kidambi2020morel,yu2020mopo} adds reward penalization to the uncertainty in model estimation, but is not robust to non-Markovian in the environment and model class misspecification.

Another approaches against overfitting is to limit the policy search space. 
A natural constraints is to thresholding the conditional action probability under behavior policy $\mu(a|s)$, such as BCQ \citep{fujimoto2019off} and POPCORN \citep{futoma2020popcorn}. However this approach does not really address the issue as in the motivating example $\mu(a|s)$ is uniform thus it provides little information on which actions lead to larger overfitting risk. In fact, the overfitting is caused by taking actions avoid the logged data purposely, instead of taking action to avoid the low conditional probability $\mu(a|s)$. Some prior work with similar ideas constraints other statistical distance between $\pi$ and $\mu$ such as BEAR-QL \citep{kumar2019stabilizing} and FDPO \citep{buckman2020importance}. More recent work PQL \citep{liu2020provably} constrain the action selection by thresholding the marginalized state action distribution, and learning the value function through a modified Bellman operator. Prior work above except POPCORN are based on learning a value function under Markov and other model assumptions, and most of their constraints are build on top of true probability. 

In the next section, we will present our method on directly optimizing the policy with importance sampling estimators, and constraining actions based on the \emph{empirical visitation in data} which is more directly related to the overfitting issue as we observed. To illustrate the limitation of prior work, in figure \ref{fig:overfitting_example_result} we show the counterfactual risk minimization regularization with or without self-normalization requires a much larger number of samples to solve the example above, compared with our algorithm proposed later. Value-based or model-based approaches will fail as well with a slight non-Markovian modification to this example in Appendix. 
% The setting does not satisfy the Markov assumption and so the value function or MDP model based approaches also fail in this setting. 
% This overfitting problem is related to the \emph{propensity overfitting} issue discussed in previous literature in contextual bandit settings. Over-weighing the weights for high-rewards contexts, as well as over-avoiding the weights for low-rewards contexts are the two sides of the same propensity (importance weights) overfitting issue: fitting the weights of context instead of the weights of actions. The norm-POEM \citep{swaminathan2015self} method use self-normalized IS estimator to avoid over-weighing high reward boundlessly. The self-normalization of weights cannot prevent over-avoiding the low-rewards contexts, which eventually also result in over-weighing high reward in a self-normalized estimator. CRM's variance penalty \citep{swaminathan2015counterfactual} method relieves the overfitting problem by the variance penalization. It combats both the unavoidable variance from reward/transition dynamics and the variance from importance weights, thus might fail to avoid the overfitting in importance weights when the variance from the environment is non-uniform. 
